Improving Adversarial Transferability via Model Alignment

Neural networks are susceptible to adversarial perturbations that are transferable across different models. In this paper, we introduce a novel model alignment technique aimed at improving a given source model's ability in generating transferable adversarial perturbations. During the alignment process, the parameters of the source model are fine-tuned to minimize an alignment loss. This loss measures the divergence in the predictions between the source model and another, independently trained model, referred to as the witness model. To understand the effect of model alignment, we conduct a geometric analysis of the resulting changes in the loss landscape. Extensive experiments on the ImageNet dataset, using a variety of model architectures, demonstrate that perturbations generated from aligned source models exhibit significantly higher transferability than those from the original source model.

==> sec/cvpr_rebuttal.tex <==
We thank all reviewers for their helpful feedback. We are pleased that the reviewers find the paper \blue{``well written''} (\rTWO/\rTHREE), and our method is \blue{``simple''} (\rthree), \blue{``novel''} (\rONE), and \blue{``likely to spark further research''} (\rone), and acknowledge the \blue{extensiveness of the experiments} (\rone/\rtwo/\rthree). Below, we respond to all reviewers' questions and concerns.

\rone/\rtwo/\rthree:
\blue{Ensemble.} We thank the reviewer for pointing out the lack of baseline ensemble comparisons. Addressing this, we implement the ensemble in logits scheme [9] following the settings in Sec.~4. Tab.~\ref{table:rebuttal_ensemble} compares transferability across four scenarios: aligned models alone~(1,~5), ensembles of source-witness models~(2,~6), ensembles of aligned models~(3,~7), and ensembles of two pairs of source-witness models~(4,~8). Results show that single aligned models yield more transferable adversarial perturbations (\textbf{AP}s) than source-witness model ensembles, and aligned model ensembles further enhance transferability, even exceeding the four-model ensembles. Additionally, our method offers the advantages of faster inference times and reduced memory storage compared to traditional ensemble approaches.

\rone/\rtwo: \blue{Overfitting.} Over-alignment can lead to overfitting, reducing the transferability of APs. For example, aligning a Res101 with a Res50 showed a drop in transferability improvement from 10.4\% to 4.2\% as epochs increased from 1 to 5. \blue{Regularization.} To mitigate overfitting, we use early stopping and limit alignment to a single epoch. In Sec. 4, we propose using an ensemble of witnesses to further lower overfitting risks. When aligning by reducing KL, we can increase the temperature in softmax to prevent exact replication of witness model predictions by the source model.

\rtwo/\rthree:
\blue{Goal and motivation.} Our goal is to transform any source model into one from which attacks generate more transferable APs.
During alignment, the source model learns to focus on a set of features that are similarly extracted by the witness model. This allows attack algorithms to more effectively exploit features common across models, leading to more transferable APs. \blue{Advantage.} A primary advantage of our method is its compatibility. Results in Tab.~6 and 7 highlight the universal compatibility with existing transfer-enhancing algorithms. Aligned models can be seamlessly integrated with off-the-shelf attacks to improve transferability. \blue{Comparing with optimization-based attacks.} We recognize there may be a misunderstanding regarding the perceived inconvenience and computational demands of the fine-tuning process in our method. It is important to clarify that our approach, due to its orthogonal nature, is not in competition with optimization-based methods, but rather complements them. This allows for combining both methods to improve transferability as shown in Tab.~6.

\rtwo: \blue{Reasons for the improved transferability.}
In Sec.~3, we demonstrate that the primary difference between the AP after alignment is the increase in the amount of low-frequency information. Previous work has shown that semantic features are low-frequency [59], and attack algorithms such as [A] are specifically designed to exploit low-frequency features to improve attack success rate. Also, we show that the loss surface becomes smoother after alignment, which is in line with previous findings that APs from flatter loss surfaces tend to be more transferable [15]. These two factors explained the improved transferability from the alignment process. \blue{Similarity of models after alignment.} To evaluate, we use KL, prediction agreement, and cosine similarity of input gradients. The latter is crucial due to its role in attack processes. 
Focusing on a Res50 aligned with a Res18 and a ViT-B with a ViT-T, 
% Focusing on Res50$\parallel$Res18 and ViT-B$\parallel$ViT-T
Tab.~\ref{table:rebuttal_similarity} shows post-alignment reductions in KL, increased cosine similarity, and improved prediction agreement.
\input{table/rebuttal_ensemble}
\input{table/rebuttal_similarity}
\blue{Training that mimics the effect of alignment. } Our analysis is empirical, observing AP differences and examining model alignment effects on the loss surface. While developing an efficient
% overfitting-proof 
optimization objective is complex and may need a theoretical framework, our approach demonstrates its feasibility.
% , marking a preliminary step in its development. 
\blue{Choosing the witness.} Entries in Tab.~2 begin with the error rate resulting from APs generated by the original source model. This is followed by the change in error rate post-alignment. Note that given a CNN-based source, employing almost any CNN as witness can yield improvements. Tab.~2 also shows the efficacy of a self-alignment strategy, as there is a consistent improvement when the source and the witness come from the same architecture.
\blue{Attack upperbound.} All target models have an error rate of 100\% under white-box PGD attack ($\epsilon=4/255$).


\rthree: \blue{“Model alignment ... already widely known”} 
The mentioned work focuses on adversarial defenses, while our approach takes a completely different direction. To our knowledge, our work is the first to specifically focus on improving a given source model’s ability to generate transferable APs through model alignment. 
\blue{Access to training samples.} The same training data used to train the source model is also used during the alignment process. No additional training samples are involved.\\

\textbf{References:}\\
\footnotesize{$[\text{A}]$ Guo et al., Low Frequency Adversarial Perturbation, UAI'19}

==> sec/eccv_rebuttal.tex <==
We thank all reviewers for positive feedback: \blue{easy to follow} (\rone/\rthree/\rfive), \blue{well-motivated} (\rone), \blue{simple yet effective} (\rone/\rthree/\rfive), and \blue{compatible with other attacks} (\rone/\rthree/\rfive). Below, we respond to all reviewers' questions.

% \vspace{-0.07cm}
\rone:
\blue{Novelty.} We wish to clarify that our method is the first to improve adversarial transferability through model alignment. 
While techniques from the distillation literature may be well-suited for alignment, this does not diminish the novelty of our approach in improving transferability.
% Even though the model alignment technique has been used for distillation, their use for improving transferability is novel.

\blue{Why KL?} 
% During alignment, the source model learns to focus on a set of features that are similarly extracted by the witness model. We implement this by minimizing the differences between the models' softmax outputs. 
In this work, we focus on output-space alignment using KL, analyze its effect from a geometric perspective, demonstrate its compatibility with other attacks, and investigate how various factors affect transferability improvement.
Given the probabilistic interpretation of model outputs, the alignment process effectively reduces the divergence between distributions. Consequently, any suitable probability divergence metric can be utilized and we opt for KL due to its widespread use. Results in Tab.~\ref{table:rebuttal_distillation} show that total variation (TV) is also effective. 
While focusing on KL, we also demonstrate the potential improvements with other metrics and formulations. Additonal discussions and results in Tab.~\ref{table:rebuttal_distillation} will be included in the revision.
% Notably, optimizing KL is equivalent to optimizing an upper bound on TV, and a similar relationship can be established with other divergence metrics [A]. 
% In this work, we focus on model output-space alignment using KL, geometrically analyze its effect, demonstrate its compatibility with other attacks, and investigate how different factors affect transferability improvement. 
% While we provide an ablation on embedding-space alignment, further exploration of this direction is considered for future work.
% Despite our focus on using KL, we also explored other metrics alignment in the embedding space., further exploration of this direction is considered for future work.

\input{table/eccv/rebuttal_distillation}
\blue{Alignment in both output and embedding spaces.} This requires optimizing the sum of two objectives, introducing an additional hyper-parameter ($\lambda$) to control their scaling: $d_q(z_s^{[q]}(x), z_w^{[q]}(x)) + \lambda d_p(z_s^{[p]}(x), z_w^{[p]}(x))$, where $p<q=l$. In Tab.~\ref{table:rebuttal_distillation}, we follow the reviewer's suggestion and combine KL with EGA and NCE ($\lambda = 1$). Results show that this further improves transferability for some targets.


\blue{Comparison with model modification-based methods.} A key advantage of our approach over model modification-based methods is its model-agnostic nature (Ln125): alignment can be applied to any model without changing its forward or backward pass. In contrast, other methods require changes, such as those seen in LinBP [16] and BPA [A], or even complete retraining from scratch [2]. Additionally, our technique can be integrated with these model modification-based methods. In Tab.~\ref{table:rebuttal_linbp}, we observe the transferability improvement of MI-FGSM-LinBP and PGD-BPA generated using the aligned Res50, when evaluated on 1000 randomly selected inputs (no selection criteria as described in Ln302).
\input{table/eccv/rebuttal_linbp}

\blue{Why are smaller models better witness?} It was observed that when aligning Res50 with Res101, the transferability improvement diminishes as epoch increases. Our hypothesis for the benefit of smaller witness models is that they focus on learning more semantically meaningful features, as larger models can memorize the dataset [B].







\rthree:
\blue{Improved transferability on defended models.} We follow the reviewer's suggestion and evaluate using a normally trained Res50 with five defense mechanisms. We adhere to the exact configuration of the defense methods as described in [59]. We also consider an adversarially trained Res50 (AT) [C]. Results in Tab.~\ref{table:rebuttal_defense} show that although the defense methods can generally reduce transferability, using the aligned model still results in a significant improvement in transferability compared to the original source model.
\input{table/eccv/rebuttal_defense}

\blue{Aligning with multiple witnesses of different architectures.} Although having more witnesses can prevent overfitting, a careful selection strategy should be considered when adopting multiple models with varying architectures. For example, accompanying a single Res50 witness model with ViT-S and IncV3 improves transferability to some target models, while the improvement decreases slightly for others.
\input{table/eccv/rebuttal_multi_witness}

\rfive:
\blue{Experiments on additional datasets.} Focusing on ImageNet is standard practice and is seen in other works [9, 28, 50]. We supplement our results with experiments on Stanford Cars (SWIN is aligned using Res50) and Food101 (Res50 is aligned using \mbox{ConvNeXt-B}). Results in Tab.~\ref{table:rebuttal_dataset} show that the improved transferability achieved through model alignment is also evident on additional datasets. 
\input{table/eccv/rebuttal_dataset}

\blue{Choosing the optimal witness model.} We infer that the reviewer is referring to the selection strategy for the witness in the second weakness. Although we do not focus on choosing the optimal witness, results in Tab.~2 show that given a CNN-based source, employing almost any CNN as witness can yield improvements. Our result also shows the efficacy of a hyper-parameter-free, self-alignment strategy. That is, the source and witness models share the same architecture and optimization procedure but are independently initialized and trained. The aligned model \textit{consistently} generates more transferable perturbation. Optimizing the choice of witness model(s) is an important direction for future work.



%\textbf{References:}\\
% \vspace{0.05cm}
\scriptsize{$[\text{A}]$Wang et al., Rethinking the backward prop. for adv. transferability, NeurIPS'23}\\
\scriptsize{$[\text{B}]$Zhang et al., Understanding DL requires rethinking generalization, ICLR'17}\\
\scriptsize{$[\text{C}]$Wong et al., Fast is better than free: Revisiting adversarial training, ICLR'20}

==> table/cvpr/compare_cosine_similarity.tex <==
\begin{table}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{1.5mm}
\small
% \footnotesize
\begin{tabular}{ ccllll } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Cos. Sim. ($10^{-2}$)}	& \multicolumn{4}{c}{Attacks}\\ \cline{3-6}
  &   & MI &	VMI &	TI & DI \\ \Xhline{2\arrayrulewidth}

\multirow{2}{*}{Res50}
& $\text{cos}(\Delta x_s, \Delta x_t)$ & 3.65 & 4.20 & 8.64 & 6.49  \\
& $\text{cos}(\Delta x_a, \Delta x_t)$ & 4.52 & 5.04 & 10.0 & 7.83   \\
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{ViT-B/16}
& $\text{cos}(\Delta x_s, \Delta x_t)$ & 4.50 & 4.61 & 9.59 & 7.34 \\ 
& $\text{cos}(\Delta x_a, \Delta x_t)$ & 5.04 & 5.18 & 10.4 & 8.37 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Comparing the cosine similarity between perturbations generated using the source model and the target model.} A noticable reduction in the cosine similarty after alignment indicates that...}
\label{table:cosine_similarity_comparison}
\end{table}

==> table/cvpr/compare_input_hessian.tex <==
\begin{table}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{6.0pt}
% \small
\small
\caption{ \textbf{Comparing the largest eigenvalue of the input Hessian on the original source model and the aligned source model.} 
Results are averaged over 1000 randomly selected data points from the ImageNet test set. The largest eigenvalue decreases significantly when evaluated on all three types of inputs.
} 
\label{table:input_hessian_comparison}
\begin{tabular}{ ccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Data}  & \multicolumn{2}{c}{\underline{Res50}} \\ 
  & Original & Aligned  \\\Xhline{2\arrayrulewidth}
Clean  	            & 4.16    & 1.25        \\ 
Gaussian-perturbed	& 4.34    & 1.27        \\
PGD-perturbed		& 0.10    & 0.05        \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
% \vspace{5mm}

\end{table}

==> table/cvpr/diff_arch.tex <==
\begin{table}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.6}
\renewcommand{\tabcolsep}{3.0pt}
%\small
\tiny
\begin{tabular}{ cccccccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Witness}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
&   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{6}{*}{Res101}
& Res50 & $39.09+14.97$ & $55.20+19.56$ & $62.92+\underline{16.97}$ & $39.80+13.50$ & $51.20+17.07$ & $35.37+10.41$ & $22.62+4.04$ & $20.02+0.98$ & $19.00+\underline{1.44}$ & $22.39+4.81$ \\
& VGG19 & $38.74+14.49$ & $53.61+14.67$ & $62.82+12.65$ & $39.13+13.37$ & $47.73+16.72$ & $35.21+10.42$ & $23.25+3.37$ & $21.27+0.65$ & $18.71+0.81$ & $22.40+4.31$ \\ 
& IncV3 & $38.89+13.76$ & $53.61+15.64$ & $60.83+18.57$ & $39.12+12.18$ & $50.49+13.65$ & $34.60+\underline{15.10}$ & $23.11+4.10$ & $20.37+1.51$ & $19.07+1.31$ & $22.98+7.39$ \\
& DN121 & $38.28+\underline{20.55}$ & $52.89+\underline{21.87}$ & $64.25+15.34$ & $38.69+\underline{15.77}$ & $50.71+\underline{22.12}$ & $33.42+14.38$ & $22.94+\underline{7.31}$ & $20.67+\underline{2.27}$ & $19.08+1.04$ & $22.69+\underline{5.56}$ \\
& ViT-B/16 & $37.28-4.72$ & $54.66-12.51$ & $63.55-20.12$ & $39.71-7.86$ & $49.87-12.93$ & $34.07-3.72$ & $24.46-1.81$ & $19.55-0.48$ & $18.59-0.34$ & $22.47-2.92$ \\
& SWIN & $37.74-2.31$ & $56.18-12.33$ & $62.29-13.61$ & $38.36-3.43$ & $49.54-7.07$ & $34.73-3.20$ & $23.77-1.45$ & $21.34-2.61$ & $18.41-1.78$ & $21.60-1.47$ \\
\Xhline{2\arrayrulewidth}
\multirow{6}{*}{VGG19}
& Res50 & $34.33+\underline{7.19}$ & $31.27+\underline{4.16}$ & $27.19+2.76$ & $80.30+5.19$ & $32.12+7.62$ & $30.26+\underline{5.91}$ & $23.08+3.45$ & $20.55+1.20$ & $19.29+1.36$ & $24.07+1.12$ \\ 
& VGG19 & $33.49+4.66$ & $29.65+2.10$ & $25.97+1.77$ & $79.37+7.30$ & $32.54+3.44$ & $31.18+1.74$ & $23.52+2.64$ & $19.99+0.68$ & $18.67+1.39$ & $23.51+0.90$ \\ 
& IncV3 & $34.53+4.91$ & $30.31+1.57$ & $27.33+1.66$ & $80.06+3.82$ & $32.20+4.94$ & $31.04+4.33$ & $23.56+2.70$ & $20.30+0.61$ & $19.50+0.61$ & $23.47+1.04$ \\ 
& DN121 & $30.80+6.35$ & $29.21+3.52$ & $23.72+\underline{5.07}$ & $78.30+\underline{10.60}$ & $31.19+\underline{10.45}$ & $29.65+5.03$ & $22.10+\underline{4.09}$ & $17.44+\underline{2.36}$ & $17.02+\underline{2.58}$ & $21.21+\underline{1.31}$ \\ 
& ViT-B/16 & $34.17-4.34$ & $30.32-5.68$ & $26.60-5.01$ & $80.01-24.66$ & $32.17-5.11$ & $30.61-3.67$ & $23.47-0.83$ & $20.70-0.37$ & $18.87+0.77$ & $23.19-2.53$ \\ 
& SWIN & $33.63-3.24$ & $29.85-5.83$ & $25.97-4.01$ & $78.54-21.91$ & $32.22-6.48$ & $30.98-4.05$ & $23.90-1.11$ & $20.16-0.73$ & $18.59+0.64$ & $23.12-2.96$ \\ 
\Xhline{2\arrayrulewidth}
\multirow{6}{*}{DN121}
& Res50 & $40.54+11.67$ & $44.15+\underline{12.96}$ & $38.40+8.37$ & $41.71+7.32$ & $61.69+11.68$ & $31.57+5.41$ & $24.30+1.69$ & $20.31+0.46$ & $18.43+1.00$ & $24.48+1.59$ \\ 
& VGG19 & $39.65+9.02$ & $45.61+6.38$ & $37.06+4.88$ & $40.54+\underline{12.34}$ & $61.27+7.87$ & $32.32+3.77$ & $23.23+2.72$ & $21.08+0.04$ & $18.25+1.22$ & $23.28+0.94$ \\ 
& IncV3 & $39.95+8.08$ & $43.11+10.50$ & $37.07+9.88$ & $39.21+9.91$ & $60.40+12.76$ & $31.72+\underline{7.24}$ & $23.40+3.81$ & $19.85+1.23$ & $18.90-0.02$ & $23.29+\underline{2.79}$ \\ 
& DN121 & $40.15+\underline{12.56}$ & $43.20+11.60$ & $37.31+\underline{10.48}$ & $41.64+9.10$ & $60.87+\underline{15.47}$ & $32.41+6.84$ & $23.88+\underline{3.99}$ & $20.04+\underline{1.59}$ & $18.22+\underline{1.24}$ & $22.96+1.86$ \\ 
& ViT-B/16 & $40.09-3.08$ & $43.85-8.43$ & $36.33-7.78$ & $40.53-6.67$ & $61.41-12.96$ & $32.64-1.78$ & $23.40+2.06$ & $20.47+1.26$ & $17.68+1.22$ & $23.89-2.78$ \\ 
& SWIN & $40.82-4.13$ & $44.15-8.57$ & $36.76-5.34$ & $41.43-6.11$ & $61.26-10.21$ & $33.05-4.64$ & $23.85+0.54$ & $20.32-0.16$ & $17.78+1.21$ & $23.44-1.88$ \\ 
\Xhline{2\arrayrulewidth}
\multirow{6}{*}{IncV3}
& Res50 & $30.18+\underline{4.92}$ & $27.19+\underline{6.59}$ & $24.48+\underline{4.27}$ & $33.23+5.49$ & $29.53+5.74$ & $53.24+4.49$ & $22.94+1.71$ & $18.49+\underline{2.26}$ & $17.85+\underline{2.74}$ & $21.22+\underline{2.23}$ \\ 
& VGG19 & $30.01+4.65$ & $27.66+2.69$ & $24.63+3.10$ & $34.71+5.70$ & $30.41+3.39$ & $52.79+4.36$ & $22.96+1.05$ & $19.25-0.54$ & $17.30+0.38$ & $21.37+0.53$ \\ 
& IncV3 & $31.24+1.78$ & $26.78+3.91$ & $24.64+3.70$ & $33.36+3.53$ & $31.26+3.06$ & $50.59+8.75$ & $22.95+1.79$ & $18.34+0.49$ & $18.00+1.41$ & $21.21+1.75$ \\ 
& DN121 & $30.64+4.50$ & $26.79+6.38$ & $25.95+2.13$ & $33.06+\underline{7.35}$ & $30.96+\underline{6.52}$ & $51.32+\underline{8.89}$ & $22.94+\underline{3.54}$ & $18.79+0.68$ & $17.90+1.41$ & $20.79+1.45$ \\ 
& ViT-B/16 & $31.65+0.47$ & $28.57-1.13$ & $24.89-2.97$ & $32.63-0.77$ & $31.56-1.35$ & $50.65-8.20$ & $23.04+2.92$ & $18.95+1.64$ & $17.84+2.07$ & $19.99-0.23$ \\ 
& SWIN & $30.34-0.49$ & $27.95-3.36$ & $25.51-3.85$ & $33.82-3.29$ & $32.19-4.54$ & $52.21-12.82$ & $23.10+0.09$ & $18.79+0.76$ & $17.42+1.13$ & $21.08-1.34$ \\ 
\Xhline{2\arrayrulewidth}
\multirow{6}{*}{ViT-B/16}
& Res50 & $23.51+\underline{17.53}$ & $20.02+12.89$ & $18.89+12.23$ & $21.41+14.83$ & $21.88+16.66$ & $21.22+15.76$ & $37.45+43.47$ & $46.01+37.17$ & $51.53+29.16$ & $21.44+21.16$ \\ 
& VGG19 & $23.51+10.89$ & $20.34+9.49$ & $18.00+9.77$ & $21.85+14.23$ & $22.44+12.65$ & $22.24+10.94$ & $35.38+39.63$ & $44.70+31.65$ & $51.43+21.30$ & $21.42+14.97$ \\ 
& IncV3 & $23.02+15.41$ & $19.62+11.87$ & $17.87+11.31$ & $21.73+\underline{15.09}$ & $21.87+14.23$ & $21.78+16.46$ & $35.16+46.07$ & $43.27+40.39$ & $52.17+28.87$ & $21.48+19.92$ \\ 
& DN121 & $22.60+17.15$ & $19.30+\underline{13.92}$ & $18.31+\underline{12.28}$ & $22.89+15.38$ & $21.75+\underline{17.68}$ & $20.55+\underline{16.96}$ & $36.55+\underline{47.36}$ & $43.70+\underline{41.88}$ & $50.15+\underline{31.22}$ & $21.44+\underline{21.87}$ \\ 
& ViT-B/16 & $21.99+5.14$ & $19.55+2.04$ & $18.43+2.07$ & $21.38+4.79$ & $22.30+2.87$ & $21.52+4.53$ & $36.90+24.04$ & $44.27+23.14$ & $50.87+21.93$ & $21.11+6.34$ \\ 
& SWIN & $23.70+6.31$ & $19.18+5.75$ & $18.31+5.92$ & $21.72+8.12$ & $21.55+7.46$ & $21.84+7.28$ & $37.20+39.11$ & $45.50+36.49$ & $51.46+28.61$ & $20.45+14.62$ \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Aligning the source model can lead to the generation of more transferable adversarial examples.} The result demonstrate the increase in error rates when adversarial examples generated from various aligned source models are applied to different target models. Our method improves the transferability of adversarial examples generated from a wide range of architectures, including both CNNs and ViTs.
}
\vspace{5mm}
\label{table:different_arch}
\end{table}

==> table/cvpr/diff_arch_imp_only.tex <==
\begin{table*}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{8.0pt}
%\small
\footnotesize
\begin{tabular}{ cccccccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Witness}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
  &   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{6}{*}{Res101}
& Res50 & 14.97 & 19.56 & \textbf{16.97} & 13.50 & 17.07 & 10.41 & 4.04 & 0.98 & \textbf{1.44} & 4.81 \\
& VGG19 & 14.49 & 14.67 & 12.65 & 13.37 & 16.72 & 10.42 & 3.37 & 0.65 & 0.81 & 4.31 \\ 
& IncV3 & 13.76 & 15.64 & 18.57 & 12.18 & 13.65 & \textbf{15.10} & 4.10 & 1.51 & 1.31 & 7.39 \\
& DN121 & \textbf{20.55} & \textbf{21.87} & 15.34 & \textbf{15.77} & \textbf{22.12} & 14.38 & \textbf{7.31} & \textbf{2.27} & 1.04 & \textbf{5.56} \\
& ViT-B/16 & -4.72 & -12.51 & -20.12 & -7.86 & -12.93 & -3.72 & -1.81 & -0.48 & -0.34 & -2.92 \\
& SWIN & -2.31 & -12.33 & -13.61 & -3.43 & -7.07 & -3.20 & -1.45 & -2.61 & -1.78 & -1.47 \\
\Xhline{2\arrayrulewidth}
\multirow{6}{*}{VGG19}
& Res50 & \textbf{7.19} & \textbf{4.16} & 2.76 & 5.19 & 7.62 & \textbf{5.91} & 3.45 & 1.20 & 1.36 & 1.12 \\
& VGG19 & 4.66 & 2.10 & 1.77 & 7.30 & 3.44 & 1.74 & 2.64 & 0.68 & 1.39 & 0.90 \\
& IncV3 & 4.91 & 1.57 & 1.66 & 3.82 & 4.94 & 4.33 & 2.70 & 0.61 & 0.61 & 1.04 \\
& DN121& 6.35 & 3.52 & \textbf{5.07} & \textbf{10.60} & \textbf{10.45} & 5.03 & \textbf{4.09} & \textbf{2.36} & \textbf{2.58} & \textbf{1.31} \\
& ViT-B/16 & -4.34 & -5.68 & -5.01 & -24.66 & -5.11 & -3.67 & -0.83 & -0.37 & 0.77 & -2.53 \\
& SWIN & -3.24 & -5.83 & -4.01 & -21.91 & -6.48 & -4.05 & -1.11 & -0.73 & 0.64 & -2.96 \\
\Xhline{2\arrayrulewidth}
\multirow{6}{*}{DN121}
& Res50 & 11.67 & \textbf{12.96} & 8.37 & 7.32 & 11.68 & 5.41 & 1.69 & 0.46 & 1.00 & 1.59 \\ 
& VGG19  & 9.02 & 6.38 & 4.88 & \textbf{12.34} & 7.87 & 3.77 & 2.72 & 0.04 & 1.22 & 0.94 \\
& IncV3  & 8.08 & 10.50 & 9.88 & 9.91 & 12.76 & \textbf{7.24} & 3.81 & 1.23 & -0.02 & \textbf{2.79} \\
& DN121  & \textbf{12.56} & 11.60 & \textbf{10.48} & 9.10 & \textbf{15.47} & 6.84 & \textbf{3.99} & \textbf{1.59} &\textbf{1.24} & 1.86 \\
& ViT-B/16 & -3.08 & -8.43 & -7.78 & -6.67 & -12.96 & -1.78 & 2.06 & 1.26 & 1.22 & -2.78 \\
& SWIN & -4.13 & -8.57 & -5.34 & -6.11 & -10.21 & -4.64 & 0.54 & -0.16 & 1.21 & -1.88 \\
\Xhline{2\arrayrulewidth}
\multirow{6}{*}{IncV3}
& Res50 & \textbf{4.92} & \textbf{6.59} & \textbf{4.27} & 5.49 & 5.74 & 4.49 & 1.71 & \textbf{2.26} & \textbf{2.74} &\textbf{ 2.23} \\
& VGG19 & 4.65 & 2.69 & 3.10 & 5.70 & 3.39 & 4.36 & 1.05 & -0.54 & 0.38 & 0.53 \\
& IncV3 & 1.78 & 3.91 & 3.70 & 3.53 & 3.06 & 8.75 & 1.79 & 0.49 & 1.41 & 1.75 \\
& DN121 & 4.50 & 6.38 & 2.13 & \textbf{7.35} & \textbf{6.52} &\textbf{ 8.89} & \textbf{3.54} & 0.68 & 1.41 & 1.45 \\
& ViT-B/16 &  0.47 & -1.13 & -2.97 & -0.77 & -1.35 & -8.20 & 2.92 & 1.64 & 2.07 & -0.23 \\
& SWIN & -0.49 & -3.36 & -3.85 & -3.29 & -4.54 & -12.82 & 0.09 & 0.76 & 1.13 & -1.34 \\
\Xhline{2\arrayrulewidth}
\multirow{6}{*}{ViT-B/16}
& Res50 & \textbf{17.53} & 12.89 & 12.23 & 14.83 & 16.66 & 15.76 & 43.47 & 37.17 & 29.16 & 21.16 \\
& VGG19 & 10.89 & 9.49 & 9.77 & 14.23 & 12.65 & 10.94 & 39.63 & 31.65 & 21.30 & 14.97 \\
& IncV3 & 15.41 & 11.87 & 11.31 & \textbf{15.09} & 14.23 & 16.46 & 46.07 & 40.39 & 28.87 & 19.92 \\
& DN121 & 17.15 & \textbf{13.92} & \textbf{12.28} & 15.38 & \textbf{17.68} & \textbf{16.96} & \textbf{47.36} & \textbf{41.88} & \textbf{31.22} & \textbf{21.87} \\
& ViT-B/16 & 5.14 & 2.04 & 2.07 & 4.79 & 2.87 & 4.53 & 24.04 & 23.14 & 21.93 & 6.34 \\
& SWIN & 6.31 & 5.75 & 5.92 & 8.12 & 7.46 & 7.28 & 39.11 & 36.49 & 28.61 & 14.62 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Aligning the source model can lead to the generation of more transferable adversarial examples.} The result demonstrate the increase in error rates when adversarial examples generated from various aligned source models are applied to different target models. Our method improves the transferability of adversarial examples generated from a wide range of architectures, including both CNNs and ViTs.
}
\label{table:different_arch}
\end{table*}

==> table/cvpr/kd_method.tex <==
\begin{table*}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.6}
\renewcommand{\tabcolsep}{3.0pt}
% \small
\tiny
\begin{tabular}{ cccccccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Method}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
  &   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{5}{*}{Res50}
& KL &$43.01+35.30$ & $61.51+\underline{26.56}$ & $51.15+25.20$ & $43.33+24.38$ & $50.74+27.86$ & $36.63+19.18$ & $26.46+5.49$ & $20.77+2.85$ & $18.17+1.61$ & $23.39+9.60$ \\ 
& RKD &$43.01+2.95$ & $61.51+2.12$ & $51.15+2.80$ & $43.33+2.78$ & $50.74+3.35$ & $36.63+4.09$ & $26.46-1.26$ & $20.77-0.53$ & $18.17-0.36$ & $23.39+0.21$ \\ 
& EGA &$43.01+\underline{35.35}$ & $61.51+23.56$ & $51.15+\underline{27.09}$ & $43.33+\underline{24.69}$ & $50.74+\underline{28.94}$ & $36.63+\underline{22.00}$ & $26.46+\underline{10.12}$ & $20.77+\underline{4.62}$ & $18.17+\underline{3.80}$ & $23.39+\underline{10.37}$ \\ 
& HINT &$43.01+5.95$ & $61.51+6.55$ & $51.15+5.27$ & $43.33+5.43$ & $50.74+9.54$ & $36.63+4.34$ & $26.46+2.55$ & $20.77-0.01$ & $18.17+1.24$ & $23.39+2.58$ \\ 
& NCE &$43.01+21.51$ & $61.51+19.25$ & $51.15+20.39$ & $43.33+16.06$ & $50.74+19.70$ & $36.63+13.29$ & $26.46+6.78$ & $20.77+3.38$ & $18.17+1.06$ & $23.39+6.73$ \\ 
\Xhline{2\arrayrulewidth}
\multirow{5}{*}{ViT-B/16}
& KL &$23.71+10.13$ & $20.34+9.71$ & $18.28+8.42$ & $22.02+10.71$ & $21.35+11.30$ & $21.44+9.89$ & $35.47+51.72$ & $44.62+44.99$ & $51.44+34.69$ & $19.44+20.01$ \\ 
& RKD &$23.71+\underline{13.40}$ & $20.34+8.47$ & $18.28+8.79$ & $22.02+11.54$ & $21.35+10.25$ & $21.44+11.37$ & $35.47+46.07$ & $44.62+43.41$ & $51.44+34.02$ & $19.44+17.51$ \\ 
& EGA &$23.71+12.55$ & $20.34+\underline{10.21}$ & $18.28+9.21$ & $22.02+11.39$ & $21.35+9.30$ & $21.44+12.05$ & $35.47+53.08$ & $44.62+44.65$ & $51.44+33.50$ & $19.44+21.40$ \\ 
& HINT &$23.71+12.78$ & $20.34+10.02$ & $18.28+\underline{9.84}$ & $22.02+\underline{12.21}$ & $21.35+\underline{12.07}$ & $21.44+\underline{12.31}$ & $35.47+\underline{53.41}$ & $44.62+\underline{47.05}$ & $51.44+\underline{38.50}$ & $19.44+\underline{25.51}$ \\ 
& NCE &$23.71+8.90$ & $20.34+8.48$ & $18.28+7.16$ & $22.02+9.00$ & $21.35+7.26$ & $21.44+7.92$ & $35.47+45.09$ & $44.62+41.84$ & $51.44+32.57$ & $19.44+15.47$ \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Improving transferability via embedding space alignment.} Both models demonstrate improved adversarian transferability when alignment is performed directly in the embedding space.}
\label{table:kd_method}
\vspace{5mm}
\end{table*}

==> table/cvpr/kd_method_imp_only.tex <==
\begin{table*}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{8.0pt}
% \small
\footnotesize
\begin{tabular}{ cccccccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Method}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
  &   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{5}{*}{Res50}
& KL & 35.30 & \textbf{26.56} & 25.20 & 24.38 & 27.86 & 19.18 & 5.49 & 2.85 & 1.61 & 9.60 \\
& RKD & 2.95 & 2.12 & 2.80 & 2.78 & 3.35 & 4.09 & -1.26 & -0.53 & -0.36 & 0.21 \\
& EGA & \textbf{35.35} & 23.56 & \textbf{27.09 }& \textbf{24.69 }& \textbf{28.94} & \textbf{22.00} & \textbf{10.12} & \textbf{4.62} & \textbf{3.80} & \textbf{10.37} \\
& HINT & 5.95 & 6.55 & 5.27 & 5.43 & 9.54 & 4.34 & 2.55 & -0.01 & 1.24 & 2.58 \\ 
& NCE & 21.51 & 19.25 & 20.39 & 16.06 & 19.70 & 13.29 & 6.78 & 3.38 & 1.06 & 6.73 \\
\Xhline{2\arrayrulewidth}
\multirow{5}{*}{ViT-B/16}
& KL & 10.13 & 9.71 & 8.42 & 10.71 & 11.30 & 9.89 & 51.72 & 44.99 & 34.69 & 20.01 \\
& RKD & \textbf{13.40} & 8.47 & 8.79 & 11.54 & 10.25 & 11.37 & 46.07 & 43.41 & 34.02 & 17.51 \\
& EGA & 12.55 & \textbf{10.21} & 9.21 & 11.39 & 9.30 & 12.05 & 53.08 & 44.65 & 33.50 & 21.40 \\
& HINT & 12.78 & 10.02 & \textbf{9.84} &\textbf{ 12.21} & \textbf{12.07} & \textbf{12.31} & \textbf{53.41} & \textbf{47.05 }& \textbf{38.50} & \textbf{25.51} \\
& NCE & 8.90 & 8.48 & 7.16 & 9.00 & 7.26 & 7.92 & 45.09 & 41.84 & 32.57 & 15.47 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Improving transferability via embedding space alignment.} Both models demonstrate improved adversarian transferability when alignment is performed directly in the embedding space.}
\label{table:kd_method}
\end{table*}

==> table/cvpr/model_capacity.tex <==
\begin{table*}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.6}
\renewcommand{\tabcolsep}{3.0pt}
%\small
\tiny
\begin{tabular}{ cccccccccccc }
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Witness}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
  &   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{2}{*}{Res18}
& Res50  & $63.81-1.94$ & $45.33+0.41$ & $36.95-0.74$ & $42.58+0.82$ & $48.65-1.24$ & $37.54-1.78$ & $27.75+0.26$ & $21.35+1.33$ & $20.55+0.42$ & $21.16+1.48$ \\ 
& Res101  & $64.39-5.13$ & $46.37-3.92$ & $37.23-2.70$ & $43.34-1.75$ & $48.49-1.39$ & $37.09-0.22$ & $27.30+0.53$ & $20.89+0.25$ & $20.60+0.03$ & $21.46+0.48$ \\ 
\hline
\multirow{2}{*}{Res50}
& Res18  & $43.01+35.30$ & $61.51+26.56$ & $51.15+25.20$ & $43.33+24.38$ & $50.74+27.86$ & $36.63+19.18$ & $26.46+5.49$ & $20.77+2.85$ & $18.17+1.61$ & $23.39+9.60$ \\ 
& Res101  & $43.91+4.27$ & $61.64+3.02$ & $52.90+3.93$ & $42.89+3.61$ & $51.11+4.41$ & $35.29+3.60$ & $25.15+1.86$ & $21.24-0.54$ & $18.04+0.14$ & $22.06+1.36$ \\ 
\hline
\multirow{2}{*}{Res101}
& Res18  & $38.59+\underline{40.64}$ & $54.05+\underline{35.11}$ & $62.99+\underline{27.78}$ & $38.68+\underline{29.63}$ & $48.67+\underline{33.20}$ & $34.17+\underline{28.42}$ & $23.41+\underline{10.10}$ & $20.22+\underline{5.70}$ & $19.15+\underline{2.37}$ & $23.41+\underline{13.99}$ \\ 
& Res50  & $39.09+14.97$ & $55.20+19.56$ & $62.92+16.97$ & $39.80+13.50$ & $51.20+17.07$ & $35.37+10.41$ & $22.62+4.04$ & $20.02+0.98$ & $19.00+1.44$ & $22.39+4.81$ \\ 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{ViT-T/16}
& ViT-S/16  & $29.13+0.30$ & $23.09+0.70$ & $20.90+1.02$ & $25.03+2.76$ & $25.38+0.54$ & $25.15+0.69$ & $63.67+7.01$ & $40.48+3.77$ & $29.99+2.92$ & $22.82+0.42$ \\ 
& ViT-B/16  & $28.40+0.86$ & $23.82-0.18$ & $21.20-1.11$ & $25.78+1.15$ & $25.53+0.47$ & $25.30+0.81$ & $64.10+5.09$ & $40.46+4.32$ & $29.25+3.55$ & $23.12-1.57$ \\ 
\hline
\multirow{2}{*}{ViT-S/16}
& ViT-T/16  & $24.50+9.64$ & $20.56+6.65$ & $18.94+6.29$ & $22.46+8.51$ & $21.83+10.66$ & $23.25+7.58$ & $46.45+40.53$ & $52.16+32.27$ & $44.85+26.10$ & $23.80+12.35$ \\ 
& ViT-B/16  & $24.04+3.10$ & $20.40+1.21$ & $18.78+2.87$ & $21.23+3.75$ & $21.98+3.19$ & $22.66+3.36$ & $48.24+19.07$ & $52.01+17.44$ & $42.86+13.81$ & $23.95+4.73$ \\ 
\hline
\multirow{2}{*}{ViT-B/16}
& ViT-T/16  & $23.71+\underline{10.13}$ & $20.34+\underline{9.71}$ & $18.28+\underline{8.42}$ & $22.02+\underline{10.71}$ & $21.35+\underline{11.30}$ & $21.44+\underline{9.89}$ & $35.47+\underline{51.72}$ & $44.62+\underline{44.99}$ & $51.44+\underline{34.69}$ & $19.44+\underline{20.01}$ \\ 
& ViT-S/16  & $22.30+7.30$ & $19.93+4.57$ & $18.46+4.53$ & $23.49+4.75$ & $22.02+6.21$ & $22.32+6.34$ & $36.56+36.47$ & $44.35+35.66$ & $50.81+29.43$ & $20.75+12.00$ \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Analyzing the impact of witness model capacity on the alignment process. } We observe a greater improvement in the transferability of adversarial perturbations when the source model is aligned with witness models of smaller capacity.}
\label{table:model_capacity}
\vspace{5mm}
\end{table*}

==> table/cvpr/model_capacity_imp_only.tex <==
\begin{table*}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{8.0pt}
%\small
\footnotesize
\begin{tabular}{ cccccccccccc }
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Witness}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
  &   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{2}{*}{Res18}
& Res50  & \textbf{-1.94} & \textbf{0.41} & \textbf{-0.74} & \textbf{0.82} & \textbf{-1.24} & -1.78 & 0.26 & \textbf{1.33} & \textbf{0.42} & \textbf{1.48} \\
& Res101 & -5.13 & -3.92 & -2.70 & -1.75 & -1.39 & \textbf{-0.22} & \textbf{0.53} & 0.25 & 0.03 & 0.48 \\
\hline
\multirow{2}{*}{Res50}
& Res18  &\textbf{ 35.30} & \textbf{26.56} & \textbf{25.20 }& \textbf{24.38} & \textbf{27.86} & \textbf{19.18} & \textbf{5.49} & \textbf{2.85} & \textbf{1.61} & \textbf{9.60} \\
& Res101 & 4.27 & 3.02 & 3.93 & 3.61 & 4.41 & 3.60 & 1.86 & -0.54 & 0.14 & 1.36 \\
\hline
\multirow{2}{*}{Res101}
& Res18  & \textbf{40.64} & \textbf{35.11} & \textbf{27.78} & \textbf{29.63} & \textbf{33.20} & \textbf{28.42} & \textbf{10.10} & \textbf{5.70} & \textbf{2.37} & \textbf{13.99} \\
% & Res18  & 40.64 & 35.11 & 27.78 & 29.63 & 33.20 & 28.42 & 10.10 & 5.70 & 2.37 & 13.99 \\
& Res50 & 14.97 & 19.56 & 16.97 & 13.50 & 17.07 & 10.41 & 4.04 & 0.98 & 1.44 & 4.81 \\
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{ViT-T/16}
& ViT-S/16  & 0.30 & \textbf{0.70} & \textbf{1.02} & \textbf{2.76} & \textbf{0.54} & 0.69 & \textbf{7.01 }& 3.77 & 2.92 & \textbf{0.42 }\\ 
& ViT-B/16 & \textbf{0.86} & -0.18 & -1.11 & 1.15 & 0.47 & \textbf{0.81} & 5.09 & \textbf{4.32} & \textbf{3.55} & -1.57 \\
\hline
\multirow{2}{*}{ViT-S/16}
& ViT-T/16  & \textbf{9.64} & \textbf{6.65} & \textbf{6.29} & \textbf{8.51} & \textbf{10.66} & \textbf{7.58} &\textbf{ 40.53} & \textbf{32.27} & \textbf{26.10 }& \textbf{12.35} \\
& ViT-B/16 & 3.10 & 1.21 & 2.87 & 3.75 & 3.19 & 3.36 & 19.07 & 17.44 & 13.81 & 4.73 \\
\hline
\multirow{2}{*}{ViT-B/16}
& ViT-T/16  & \textbf{10.13} & \textbf{9.71} & \textbf{8.42} & \textbf{10.71} & \textbf{11.30} & \textbf{9.89} & \textbf{51.72} & \textbf{44.99} & \textbf{34.69} & \textbf{20.01}\\
% & ViT-T/16  & 10.13 & 9.71 & 8.42 & 10.71 & 11.30 & 9.89 & 51.72 & 44.99 & 34.69 & 20.01\\
& ViT-S/16  & 7.30 & 4.57 & 4.53 & 4.75 & 6.21 & 6.34 & 36.47 & 35.66 & 29.43 & 12.00 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Analyzing the impact of witness model capacity on the alignment process. } We observe a greater improvement in the transferability of adversarial perturbations when the source model is aligned with witness models of smaller capacity.}
\label{table:model_capacity}
\end{table*}

==> table/cvpr/noise_type.tex <==
\begin{table*}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{1.5mm}
\small
% \footnotesize
\begin{tabular}{ ccllllllllll } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Noise type}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
  &   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{3}{*}{Res50}
& None & 35.30 & 26.56 & 25.20 & 24.38 & 27.86 & 19.18 & 5.49 & 2.85 & 1.61 & 9.60 \\
& Rand & 32.75 & 26.19 & 27.91 & 23.04 & 28.06 & 22.76 & 6.19 & 4.90 & 3.55 & 6.91 \\
& PGD & 41.746 & 26.52 & 28.59 & 26.30 & 31.70 & 35.23 & 27.35 & 21.28 & 14.01 & 19.24 \\
\Xhline{2\arrayrulewidth}
\multirow{3}{*}{ViT-B/16}
& None & 10.13 & 9.71 & 8.42 & 10.71 & 11.30 & 9.89 & 51.72 & 44.99 & 34.69 & 20.01 \\ 
& Rand & 10.685 & 9.86 & 8.71 & 12.78 & 10.28 & 10.60 & 50.78 & 46.20 & 37.62 & 20.31 \\
& PGD & 22.104 & 20.173 & 18.39 & 20.80 & 20.20 & 20.73 & 58.63 & 52.80 & 46.65 & 30.38 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{alignment based on perturbed training dataset}}
\label{table:noise_type}
\end{table*}

==> table/cvpr/num_witness.tex <==
\begin{table*}[th]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.6}
\renewcommand{\tabcolsep}{3.0pt}
% \small
\tiny
\begin{tabular}{ cllllllllll }
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{\# Witness}	& \multicolumn{10}{c}{Target}\\ \cline{2-11}
 &Res18 & Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}
1& $43.01+35.30$ & $61.51+26.56$ & $51.15+25.20$ & $43.33+24.38$ & $50.74+27.86$ & $36.63+19.18$ & $26.46+5.49$ & $20.77+2.85$ & $18.17+1.61$ & $23.39+9.60$ \\
2&$43.01+35.01$ & $61.51+\underline{27.83}$ & $51.15+24.82$ & $43.33+24.50$ & $50.74+27.88$ & $36.63+19.31$ & $26.46+8.28$ & $20.77+3.82$ & $18.17+1.19$ & $23.39+10.67$ \\
3&$43.01+34.69$ & $61.51+27.69$ & $51.15+27.39$ & $43.33+24.37$ & $50.74+\underline{29.44}$ & $36.63+21.51$ & $26.46+8.19$ & $20.77+4.49$ & $18.17+3.27$ & $23.39+11.74$ \\
4&$43.01+\underline{35.57}$ & $61.51+27.63$ & $51.15+\underline{27.94}$ & $43.33+\underline{25.12}$ & $50.74+28.61$ & $36.63+\underline{21.81}$ & $26.46+\underline{8.29}$ & $20.77+\underline{5.00}$ & $18.17+\underline{3.78}$ & $23.39+\underline{12.15}$ \\

\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Aligning the Res50 source model with multiple Res18 as witness models.} Using an increasing number of Res18 witness models during the alignment process results in a modest improvement in transferability for adversarial examples generated from the aligned Res50.
% 
This result suggests that simply quadrupling the number of witness models, without considering their diversity, does not lead to a proportional improvement in transferability. }
\label{table:num_witness}
\end{table*}

==> table/cvpr/num_witness_imp_only.tex <==
\begin{table*}[th]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{8pt}
% \small
\footnotesize
\begin{tabular}{ cllllllllll }
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{\# Witness}	& \multicolumn{10}{c}{Target}\\ \cline{2-11}
 &Res18 & Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}
1 &35.30 & 26.56 & 25.20 & 24.38 & 27.86 & 19.18 & 5.49 & 2.85 & 1.61 & 9.60 \\
2 &35.01 & 27.83 & 24.82 & 24.50 & 27.88 & 19.31 & 8.28 & 3.82 & 1.19 & 10.67 \\
3 &34.69 & 27.69 & 27.39 & 24.37 & 29.44 & 21.51 & 8.19 & 4.49 & 3.27 & 11.74 \\
4 &35.57 & 27.63 & 27.24 & 25.12 & 28.61 & 21.81 & 8.29 & 5.00 & 3.78 & 12.15 \\

\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Aligning the Res50 source model with multiple Res18 as witness models.} Using an increasing number of Res18 witness models during the alignment process results in further improved transferability for adversarial examples generated from the aligned Res50. }
\label{table:num_witness}
\end{table*}

==> table/cvpr/orthogonality.tex <==

\begin{table*}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.6}
\renewcommand{\tabcolsep}{3.0pt}
% \small
\tiny
\begin{tabular}{ cccccccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Attack}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
  &   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{7}{*}{Res50}
% \multirow{7}{*}{\rotatebox[origin=c]{90}{Res50}}
& MI & $75.54+20.23$ & $88.62+9.63$ & $83.13+12.77$ & $71.46+19.97$ & $79.60+16.31$ & $59.08+22.22$ & $38.30+16.04$ & $31.90+8.34$ & $25.19+7.87$ & $37.04+16.02$ \\ 
& NI & $59.71+21.99$ & $68.07+16.14$ & $60.13+17.39$ & $56.30+19.14$ & $59.56+19.90$ & $46.45+15.59$ & $33.32+10.53$ & $28.62+6.04$ & $26.66+3.62$ & $28.62+8.41$ \\ 
& VMI & $85.26+12.70$ & $96.79+2.34$ & $91.06+6.74$ & $83.16+13.13$ & $88.09+9.72$ & $71.98+16.68$ & $45.31+19.00$ & $38.45+12.12$ & $29.62+8.32$ & $49.13+15.45$ \\ 
& VNI & $86.92+11.18$ & $96.50+3.22$ & $92.07+6.03$ & $85.64+11.36$ & $90.47+8.21$ & $73.60+16.40$ & $44.71+18.43$ & $36.46+10.78$ & $29.15+8.58$ & $46.64+16.75$ \\ 
& SINI & $67.43+17.05$ & $74.16+9.08$ & $65.27+9.24$ & $61.73+11.87$ & $65.82+13.34$ & $53.74+11.96$ & $35.40+7.50$ & $30.23+1.05$ & $26.07+3.03$ & $30.59+5.29$ \\ 
& TI & $71.31+21.67$ & $84.98+10.66$ & $70.69+16.42$ & $64.87+20.13$ & $73.95+16.85$ & $53.13+19.18$ & $40.34+14.84$ & $30.06+10.78$ & $25.58+7.59$ & $30.00+11.71$ \\ 
& DI & $87.95+11.03$ & $95.92+3.49$ & $91.93+5.87$ & $82.12+15.88$ & $90.02+9.40$ & $77.78+15.45$ & $43.11+21.66$ & $33.52+14.47$ & $27.48+8.69$ & $43.20+21.83$ \\ 

\Xhline{2\arrayrulewidth}
\multirow{7}{*}{ViT-B/16}
% \multirow{7}{*}{\rotatebox[origin=c]{90}{ViT-B/16}}
& MI & $33.73+15.60$ & $31.15+13.05$ & $29.57+11.33$ & $35.24+12.06$ & $32.29+13.51$ & $33.97+11.85$ & $57.70+35.78$ & $66.18+29.45$ & $71.48+24.13$ & $33.57+20.87$ \\ 
& NI & $35.10+6.93$ & $31.44+6.05$ & $28.44+3.03$ & $35.58+4.58$ & $31.93+7.44$ & $33.67+5.70$ & $47.43+29.05$ & $50.18+21.59$ & $53.55+17.73$ & $30.69+8.60$ \\ 
& VMI & $35.59+18.65$ & $32.83+16.35$ & $29.13+16.65$ & $37.82+14.72$ & $34.55+16.12$ & $34.42+15.15$ & $62.41+33.14$ & $72.53+24.72$ & $77.20+19.14$ & $37.63+21.75$ \\ 
& VNI & $33.99+22.45$ & $32.93+17.56$ & $29.11+19.49$ & $37.19+17.16$ & $32.59+19.92$ & $33.19+20.83$ & $65.01+32.18$ & $74.13+23.26$ & $80.07+17.44$ & $38.19+21.89$ \\ 
& SINI & $36.68+11.40$ & $33.53+6.72$ & $29.47+4.58$ & $36.56+7.49$ & $33.12+9.63$ & $35.87+9.70$ & $58.50+23.57$ & $58.49+19.37$ & $62.07+9.97$ & $33.02+10.26$ \\ 
& TI & $36.85+29.96$ & $35.61+25.93$ & $28.10+23.31$ & $32.74+24.05$ & $35.48+25.98$ & $32.99+21.31$ & $55.88+40.38$ & $64.79+30.79$ & $67.16+27.23$ & $32.50+25.52$ \\ 
& DI & $41.75+30.79$ & $38.17+30.54$ & $32.53+30.23$ & $39.03+30.42$ & $41.40+26.69$ & $38.62+30.51$ & $68.50+29.43$ & $79.68+17.99$ & $84.10+13.70$ & $42.09+29.79$ \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Compatibility of model alignment with different attack algorithms. } We consider a range of attack methods, including those based on optimization and data augmentation. The results demonstrate that all considered attack algorithms can benefit from the alignment process.}
\label{table:orthogonality}
\end{table*}

==> table/cvpr/orthogonality_imp_only.tex <==

\begin{table*}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{8.0pt}
% \small
\footnotesize
\begin{tabular}{ cccccccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Attack}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
  &   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{7}{*}{Res50}
% & PGD & 25.70 & 12.53 & 19.36 & 24.74 & 18.91 & 22.31 & 13.68 & 7.58 & 6.12 & 15.14 \\
& MI & 20.225 & 9.63 & 12.77 & 19.97 & 16.31 & 22.22 & 16.04 & 8.34 & 7.87 & 16.02 \\ 
& NI & 21.985 & 16.14 & 17.39 & 19.14 & 19.90 & 15.59 & 10.53 & 6.04 & 3.62 & 8.41 \\
& VMI & 12.701 & 2.34 & 6.74 & 13.13 & 9.72 & 16.68 & 19.00 & 12.12 & 8.32 & 15.45 \\
& VNI & 11.184 & 3.22 & 6.03 & 11.36 & 8.21 & 16.40 & 18.43 & 10.78 & 8.58 & 16.75 \\ 
& SINI& 17.049 & 9.08 & 9.24 & 11.87 & 13.34 & 11.96 & 7.50 & 1.05 & 3.03 & 5.29 \\
& TI & 21.67 & 10.66 & 16.42 & 20.13 & 16.85 & 19.18 & 14.84 & 10.78 & 7.59 & 11.71 \\ 
& DI & 11.034 & 3.49 & 5.87 & 15.88 & 9.40 & 15.45 & 21.66 & 14.47 & 8.69 & 21.83 \\ 
\Xhline{2\arrayrulewidth}
\multirow{7}{*}{ViT-B/16}
% & PGD & 10.20 & 9.50 & 9.44 & 10.37 & 10.16 & 10.03 & 50.22 & 44.82 & 34.48 & 17.88 \\ 
& MI & 12.918 & 12.08 & 10.25 & 10.46 & 11.59 & 9.98 & 46.13 & 39.93 & 29.92 & 19.77 \\
& NI & 5.28 & 6.69 & 5.77 & 6.34 & 5.60 & 6.41 & 31.35 & 25.08 & 16.33 & 9.41 \\
& VMI & 12.881 & 12.67 & 11.07 & 12.45 & 13.19 & 13.15 & 45.81 & 38.35 & 29.52 & 20.80 \\
& VNI & 16.014 & 12.93 & 11.68 & 13.62 & 13.37 & 13.33 & 42.60 & 35.51 & 26.09 & 21.68 \\
& SINI& 7.811 & 7.95 & 4.75 & 6.59 & 5.35 & 6.97 & 28.58 & 18.50 & 7.18 & 7.47 \\
& TI & 15.544 & 14.88 & 10.26 & 12.69 & 14.16 & 10.02 & 38.30 & 33.32 & 26.42 & 15.50 \\
& DI & 20.821 & 20.21 & 18.61 & 18.36 & 16.44 & 22.74 & 41.05 & 35.44 & 24.33 & 25.57 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Compatibility of model alignment with different attack algorithms. } We consider a range of attack methods, including those based on optimization and data augmentation. The results demonstrate that all considered attack algorithms can benefit from the alignment process.}
\label{table:orthogonality}
\end{table*}

==> table/cvpr/rebuttal_ensemble.tex <==
\begin{table}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{0.9}
\renewcommand{\tabcolsep}{0.7mm}
% \small
\tiny
\begin{tabular}{ cccccccccccc }
\Xhline{2\arrayrulewidth}
  &\multirow{2}{*}{\underline{Source}}  & \multicolumn{10}{c}{Target}\\ \cline{3-12}
  & & Res18 & Res50 &  Res101 & VGG19& DN121& IncV3& ViT-T/16& ViT-S/16& ViT-B/16& SWIN \\ \Xhline{2\arrayrulewidth}
 1 & Res50* & \textbf{65.71} & \textbf{79.75}  & \textbf{63.67}  & \textbf{57.77}  & \textbf{71.23}  & \textbf{44.78} & \textbf{13.64}  & \textbf{7.31 }& \textbf{4.86 }& \textbf{18.84}  \\
 2 & Res50 + Res18  & 62.03 & 63.86  & 48.10  & 48.08  & 55.13  & 34.17 & 10.69  & 5.64 & 4.64 & 11.97  \\ \hline
   3 &  2$\times$Res50*  & \textbf{86.51} & \textbf{95.64}  & \textbf{87.17}  & \textbf{78.01}  & \textbf{89.01}  & \textbf{63.83} & \textbf{21.56}  & \textbf{10.53}  & \textbf{8.02 }& \textbf{27.13}  \\ 
4&  2$\times$(Res50 + Res18)  & 82.96 & 85.09  & 75.08  & 66.77  & 78.73  & 51.33 & 14.97  & 7.31 & 4.95 & 19.81  \\
\Xhline{2\arrayrulewidth}
5&  ViT-B*  & \textbf{18.68} & \textbf{12.96}  & \textbf{11.75}  & \textbf{17.03}  & \textbf{16.53}  & \textbf{17.44} & \textbf{85.24}  & \textbf{82.87}  & \textbf{82.69}  & \textbf{24.31}  \\
 6 & ViT-B + ViT-T  & 8.67  & 5.21 & 4.34 & 8.52 & 7.78 & 9.20  & 57.02  & 43.78  & 42.86  & 10.36  \\ \hline
7 &2$\times$ViT-B*  & \textbf{23.65} & \textbf{18.07}  & \textbf{15.85}  & \textbf{22.95}  & \textbf{19.81}  & \textbf{22.05} & \textbf{95.08}  & \textbf{95.52}  & \textbf{93.39}  & \textbf{35.27}  \\
8 & 2$\times$(ViT-B + ViT-T)  & 11.96 & 9.47 & 8.26 & 11.01  & 10.05  & 11.69 & 79.69  & 68.94  & 65.05  & 17.95 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\vspace{-19pt}
\caption{\scriptsize{More transferable APs from using aligned models alone or in an ensemble.}}
\label{table:rebuttal_ensemble}
\vspace{-11pt}
\end{table}

==> table/cvpr/rebuttal_similarity.tex <==
\begin{table}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{0.9}
\renewcommand{\tabcolsep}{1.2mm}
% \small
\tiny
% \vspace{-2pt}
\begin{tabular}{ ccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Model}  & \multicolumn{2}{c}{\underline{KL}} & \multicolumn{2}{c}{\underline{Agreement in prediction}} & \multicolumn{2}{c}{\underline{Cosine similarity bw input gradients}}\\ 
            & Before & After & Before & After & Before & After\\\Xhline{2\arrayrulewidth}
Res50  	    & 0.63    & 0.31   & 80.7\%    & 82.4\% & 0.043    & 0.096     \\ 
ViT-B	    & 0.75    & 0.24   & 78.9\%    & 85.0\% & 0.026    & 0.063    \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\vspace{-19pt}
\caption{\footnotesize{Similarity between models after alignment.}}
\label{table:rebuttal_similarity}
\vspace{-22pt}
\end{table}

==> table/eccv/kd_method.tex <==
\begin{table*}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.2}
\renewcommand{\tabcolsep}{2.0pt}
% \small
\tiny
\caption{ \textbf{Improving transferability via embedding space alignment.} We focus on Res50 and ViT-B/16 as source models, and they are aligned using a Res18 and a ViT-T/16 as the witness model, respectively. Both models demonstrate improved adversarial transferability when alignment is performed directly in the embedding space.}
\label{table:kd_method}
\begin{tabular}{ cccccccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Method}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
  &   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{6}{*}{Res50}
& n/a 								& $44.52$	& $61.51$	& $53.01$	& $43.47$	& $50.59$	& $36.05$	& $25.58$	& $21.54$	& $18.86$	& $22.65$ \\
& KL 								& $+35.30$	& \gc$+26.56$	& $+25.20$	& $+24.38$	& $+27.86$	& $+19.18$	& $+5.49$	& $+2.85$	& $+1.61$	& $+9.60$ \\
& RKD~\cite{park2019relational} 	& $+2.95$	& $+2.12$	& $+2.80$	& $+2.78$	& $+3.35$	& $+4.09$	& $-1.26$	& $-0.53$	& $-0.36$	& $+0.21$ \\
& EGA~\cite{ma2022distilling} 		& \gc$+35.35$	& $+23.56$	& \gc$+27.09$	& \gc$+24.69$	& \gc$+28.94$	& \gc$+22.00$	& \gc$+10.12$	& \gc$+4.62$	& \gc$+3.80$	& \gc$+10.37$ \\
& HINT~\cite{romero2014fitnets} 	& $+5.95$	& $+6.55$	& $+5.27$	& $+5.43$	& $+9.54$	& $+4.34$	& $+2.55$	& $-0.01$	& $+1.24$	& $+2.58$ \\
& NCE~\cite{chen2021distilling} 	& $+21.51$	& $+19.25$	& $+20.39$	& $+16.06$	& $+19.70$	& $+13.29$	& $+6.78$	& $+3.38$	& $+1.06$	& $+6.73$ \\
\Xhline{2\arrayrulewidth}
\multirow{6}{*}{ViT-B/16}
& n/a 								& $23.05$	& $19.67$	& $18.30$	& $21.83$	& $21.96$	& $21.52$	& $36.44$	& $44.58$	& $51.27$	& $21.22$ \\
& KL 								& $+10.13$	& $+9.71$	& $+8.42$	& $+10.71$	& $+11.30$	& $+9.89$	& $+51.72$	& $+44.99$	& $+34.69$	& $+20.01$ \\
& RKD~\cite{park2019relational} 	& \gc$+13.40$	& $+8.47$	& $+8.79$	& $+11.54$	& $+10.25$	& $+11.37$	& $+46.07$	& $+43.41$	& $+34.02$	& $+17.51$ \\
& EGA~\cite{ma2022distilling} 		& $+12.55$	& \gc$+10.21$	& $+9.21$	& $+11.39$	& $+9.30$	& $+12.05$	& $+53.08$	& $+44.65$	& $+33.50$	& $+21.40$ \\
& HINT~\cite{romero2014fitnets} 	& $+12.78$	& $+10.02$	& \gc$+9.84$	& \gc$+12.21$	& \gc$+12.07$	& \gc$+12.31$	& \gc$+53.41$	& \gc$+47.05$	& \gc$+38.50$	& \gc$+25.51$ \\
& NCE~\cite{chen2021distilling} 	& $+8.90$	& $+8.48$	& $+7.16$	& $+9.00$	& $+7.26$	& $+7.92$	& $+45.09$	& $+41.84$	& $+32.57$	& $+15.47$ \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
% \vspace{-0.6cm}
\end{table*}

==> table/eccv/orthogonality_part2.tex <==
\begin{table*}[t]
\begin{center}
% \renewcommand{\arraystretch}{\TabResultRowSpace}
\renewcommand{\arraystretch}{1.3}
\renewcommand{\tabcolsep}{2.0pt}
% \small
\tiny
\begin{tabular}{ cccccccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}		&	\multirow{2}{*}{Attack}	& \multicolumn{10}{c}{Target}\\ \cline{3-12}
  &   & Res18 &	Res50 &	Res101 &	VGG19&	DN121&	IncV3&	ViT-T/16&	ViT-S/16&	ViT-B/16&	SWIN \\ \Xhline{2\arrayrulewidth}

\multirow{7}{*}{Res50}
% \multirow{7}{*}{\rotatebox[origin=c]{90}{Res50}}
& MI & $75.54+20.23$ & $88.62+9.63$ & $83.13+12.77$ & $71.46+19.97$ & $79.60+16.31$ & $59.08+22.22$ & $38.30+16.04$ & $31.90+8.34$ & $25.19+7.87$ & $37.04+16.02$ \\ 
& NI & $59.71+21.99$ & $68.07+16.14$ & $60.13+17.39$ & $56.30+19.14$ & $59.56+19.90$ & $46.45+15.59$ & $33.32+10.53$ & $28.62+6.04$ & $26.66+3.62$ & $28.62+8.41$ \\ 
& VMI & $85.26+12.70$ & $96.79+2.34$ & $91.06+6.74$ & $83.16+13.13$ & $88.09+9.72$ & $71.98+16.68$ & $45.31+19.00$ & $38.45+12.12$ & $29.62+8.32$ & $49.13+15.45$ \\ 
& VNI & $86.92+11.18$ & $96.50+3.22$ & $92.07+6.03$ & $85.64+11.36$ & $90.47+8.21$ & $73.60+16.40$ & $44.71+18.43$ & $36.46+10.78$ & $29.15+8.58$ & $46.64+16.75$ \\ 
& SINI & $67.43+17.05$ & $74.16+9.08$ & $65.27+9.24$ & $61.73+11.87$ & $65.82+13.34$ & $53.74+11.96$ & $35.40+7.50$ & $30.23+1.05$ & $26.07+3.03$ & $30.59+5.29$ \\ 
& TI & $71.31+21.67$ & $84.98+10.66$ & $70.69+16.42$ & $64.87+20.13$ & $73.95+16.85$ & $53.13+19.18$ & $40.34+14.84$ & $30.06+10.78$ & $25.58+7.59$ & $30.00+11.71$ \\ 
& DI & $87.95+11.03$ & $95.92+3.49$ & $91.93+5.87$ & $82.12+15.88$ & $90.02+9.40$ & $77.78+15.45$ & $43.11+21.66$ & $33.52+14.47$ & $27.48+8.69$ & $43.20+21.83$ \\ 

\Xhline{2\arrayrulewidth}
\multirow{7}{*}{ViT-B/16}
% \multirow{7}{*}{\rotatebox[origin=c]{90}{ViT-B/16}}
& MI & $33.73+15.60$ & $31.15+13.05$ & $29.57+11.33$ & $35.24+12.06$ & $32.29+13.51$ & $33.97+11.85$ & $57.70+35.78$ & $66.18+29.45$ & $71.48+24.13$ & $33.57+20.87$ \\ 
& NI & $35.10+6.93$ & $31.44+6.05$ & $28.44+3.03$ & $35.58+4.58$ & $31.93+7.44$ & $33.67+5.70$ & $47.43+29.05$ & $50.18+21.59$ & $53.55+17.73$ & $30.69+8.60$ \\ 
& VMI & $35.59+18.65$ & $32.83+16.35$ & $29.13+16.65$ & $37.82+14.72$ & $34.55+16.12$ & $34.42+15.15$ & $62.41+33.14$ & $72.53+24.72$ & $77.20+19.14$ & $37.63+21.75$ \\ 
& VNI & $33.99+22.45$ & $32.93+17.56$ & $29.11+19.49$ & $37.19+17.16$ & $32.59+19.92$ & $33.19+20.83$ & $65.01+32.18$ & $74.13+23.26$ & $80.07+17.44$ & $38.19+21.89$ \\ 
& SINI & $36.68+11.40$ & $33.53+6.72$ & $29.47+4.58$ & $36.56+7.49$ & $33.12+9.63$ & $35.87+9.70$ & $58.50+23.57$ & $58.49+19.37$ & $62.07+9.97$ & $33.02+10.26$ \\ 
& TI & $36.85+29.96$ & $35.61+25.93$ & $28.10+23.31$ & $32.74+24.05$ & $35.48+25.98$ & $32.99+21.31$ & $55.88+40.38$ & $64.79+30.79$ & $67.16+27.23$ & $32.50+25.52$ \\ 
& DI & $41.75+30.79$ & $38.17+30.54$ & $32.53+30.23$ & $39.03+30.42$ & $41.40+26.69$ & $38.62+30.51$ & $68.50+29.43$ & $79.68+17.99$ & $84.10+13.70$ & $42.09+29.79$ \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\caption{ \textbf{Compatibility of model alignment with different attack algorithms. } We consider a range of attack methods, including those based on optimization and data augmentation. The results demonstrate that all considered attack algorithms can benefit from the alignment process.}
\label{table:orthogonality}
\end{table*}

==> table/eccv/rebuttal_dataset.tex <==
\begin{table}[h]
\captionsetup{font=scriptsize}
\begin{center}
\renewcommand{\arraystretch}{1}
\renewcommand{\tabcolsep}{0.7mm}
\scriptsize
\vspace{-10pt}
\begin{tabular}{ cccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Source}  & \multicolumn{2}{c}{Target} \\ \cline{3-4}
                         & & ConvNeXt-B & ViT-B \\\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Stanford Cars} &SWIN  	    & 68.77    & 17.6      \\ 
                               &SWIN*	     & \gc{88.89}    & \gc{50.67}      \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\quad
\begin{tabular}{ cccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Source}  & \multicolumn{2}{c}{Target} \\ \cline{3-4}
                         & & SWIN & ViT-B \\\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Food101} &Res50  	    & 26.67    & 12.36      \\ 
                         &Res50*	       & \gc{31.88}    & \gc{16.16}      \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\vspace{-20pt}
\caption{Generalizability of model alignment on other datasets.}
\label{table:rebuttal_dataset}
\vspace{-13pt}
\end{table}

==> table/eccv/rebuttal_defense.tex <==
\begin{table}[h]
\captionsetup{font=scriptsize}
\begin{center}
\renewcommand{\arraystretch}{1}
\renewcommand{\tabcolsep}{1.1mm}
\scriptsize
\vspace{-10pt}
\begin{tabular}{ cccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Source}  & \multicolumn{7}{c}{Defense} \\  \cline{2-8}
                         & n/a & AT & Bit-Red & JPEG & FD & RS & NRP \\\Xhline{2\arrayrulewidth}
Res50  	    & 61.51 & 48.06 & 49.22	& 38.81	& 43.77	& 35.41	& 33.01  \\ 
Res50*	    & \gc{88.07} & \gc{52.15}	& \gc{54.70}	& \gc{53.03}	& \gc{50.59}	& \gc{43.99}	& \gc{41.19}  \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\vspace{-20pt}
\caption{Improved transferability on Res50 with defense methods.}
\label{table:rebuttal_defense}
\vspace{-13pt}
\end{table}

==> table/eccv/rebuttal_distillation.tex <==
\begin{table}[h]
\captionsetup{font=scriptsize}
\begin{center}
\renewcommand{\arraystretch}{1}
\renewcommand{\tabcolsep}{1.1mm}
\scriptsize
\vspace{-10pt}
% \begin{tabular}{ ccccccccccc } 
% \Xhline{2\arrayrulewidth}
% \multirow{2}{*}{Method}  & \multicolumn{10}{c}{Target} \\ \cline{2-11}
%         & Res18	&Res50  &Res101 &VGG19	&DN121	&IncV3	&ViT-T	&ViT-S	&ViT-B	&SWIN \\\Xhline{2\arrayrulewidth}
% KL  	& 79.82	&88.07	&78.20  &67.85	&78.45	&55.22	&31.07	&24.39	&20.48	&32.25     \\ 
% TV	    & 70.56 &81.42	&64.88  &60.87	&71.24	&51.98	&31.27	&23.25	&19.71	&28.44     \\\hline
% EGA     & 79.87	&85.07	&80.10	&68.15	&79.53	&58.05	&35.70	&26.16	&22.66	&33.02     \\
% KL+EGA  & \gc{80.26}	&\gc{87.61}	&76.23	&\gc{72.36}	&\gc{80.17}	&56.10	&34.19	&25.35	&20.67	&\gc{36.69}     \\\hline
% NCE     & 66.04	&80.76	&73.40	&59.52	&70.29	&49.33	&32.36	&24.92	&19.92	&29.38     \\ 
% KL+NCE  & \gc{75.87}	&\gc{85.96}	&73.12	&\gc{66.08}	&\gc{77.72}	&\gc{55.11}	&\gc{34.06}	&23.04	&\gc{21.22}	&\gc{34.82}     \\ 
% \Xhline{2\arrayrulewidth}
% \end{tabular}
\begin{tabular}{ ccccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Method}  & \multicolumn{8}{c}{Target} \\ \cline{2-9}
        & Res18	&Res50  &VGG19	&DN121	&IncV3	&ViT-T	&ViT-S	&SWIN \\\Xhline{2\arrayrulewidth}
KL  	& 79.82	&88.07	&67.85	&78.45	&55.22	&31.07	&24.39	&32.25     \\ 
TV	    & 70.56 &81.42	&60.87	&71.24	&51.98	&31.27	&23.25	&28.44     \\\hline
EGA     & 79.87	&85.07	&68.15	&79.53	&58.05	&35.70	&26.16	&33.02     \\
KL+EGA  & \gc{80.26}	&\gc{87.61}	&\gc{72.36}	&\gc{80.17}	&56.10	&34.19	&25.35	&\gc{36.69}     \\\hline
NCE     & 66.04	&80.76	&59.52	&70.29	&49.33	&32.36	&24.92	&29.38     \\ 
KL+NCE  & \gc{75.87}	&\gc{85.96}	&\gc{66.08}	&\gc{77.72}	&\gc{55.11}	&\gc{34.06}	&23.04	&\gc{34.82}     \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\vspace{-20pt}
\caption{Model alignment with different objectives.}
\label{table:rebuttal_distillation}
\vspace{-15pt}
\end{table}

==> table/eccv/rebuttal_linbp.tex <==
\begin{table}[h]
\captionsetup{font=scriptsize}
\begin{center}
\renewcommand{\arraystretch}{1}
\renewcommand{\tabcolsep}{1.1mm}
\scriptsize
\vspace{-20pt}

% V1
% \begin{tabular}{ ccccccccccc } 
% \Xhline{2\arrayrulewidth}
% \multirow{2}{*}{Source}  & \multicolumn{10}{c}{Target} \\ \cline{2-11}
%                         & Res18	&Res50  &Res101 &VGG19	&DN121	&IncV3	&ViT-T	&ViT-S	&ViT-B	&SWIN \\\Xhline{2\arrayrulewidth}
% Res50  	                & 87.89	&93.55	&87.50	&84.08	&88.57	&71.19	&43.16	&33.50	&28.71	&46.19     \\ 
% Res50*	                & \gc{97.27}	&\gc{96.27}	&\gc{93.75}	&\gc{93.07}	&\gc{95.61}	&\gc{86.04}	&\gc{56.25}	&\gc{41.02}	&\gc{34.08}	&\gc{57.71}     \\
% \Xhline{2\arrayrulewidth}
% \end{tabular}

% V2
% \begin{tabular}{ ccccccccc } 
% \Xhline{2\arrayrulewidth}
% \multirow{2}{*}{Source}  & \multicolumn{8}{c}{Target} \\ \cline{2-9}
%                         & Res18	&Res50  &VGG19	&DN121	&IncV3	&ViT-T	&ViT-S	&SWIN \\\Xhline{2\arrayrulewidth}
% Res50  	                & 87.89	&93.55	&84.08	&88.57	&71.19	&43.16	&33.50	&46.19     \\ 
% Res50*	                & \gc{97.27}	&\gc{96.27}	&\gc{93.07}	&\gc{95.61}	&\gc{86.04}	&\gc{56.25}	&\gc{41.02}	&\gc{57.71}     \\
% \Xhline{2\arrayrulewidth}
% \end{tabular}

\begin{tabular}{ ccccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Attack} &\multirow{2}{*}{Source}  & \multicolumn{7}{c}{Target} \\ \cline{3-9}
                        &       & Res18	&Res50  &VGG19	&DN121	&IncV3	&ViT-T	&SWIN \\\Xhline{2\arrayrulewidth}
\multirow{2}{*}{LinBP}  &Res50  & 87.89	&93.55	&84.08	&88.57	&71.19	&43.16	&46.19     \\ 
                        &Res50*	& \gc{97.27}	&\gc{96.27}	&\gc{93.07}	&\gc{95.61}	&\gc{86.04}	&\gc{56.25}	&\gc{57.71}     \\\hline
\multirow{2}{*}{BPA}    &Res50  & 51.06	&63.98	&51.54	&58.24	&34.02	&12.0	&11.04     \\ 
                        &Res50*	& \gc{76.76}	&\gc{81.98}	&\gc{70.62}	&\gc{77.98}	&\gc{53.18}	&\gc{19.3}	&\gc{20.06}     \\
\Xhline{2\arrayrulewidth}
\end{tabular}

\end{center}
\vspace{-20pt}
\caption{Model alignment can be integrated with model modification-based methods.}
\label{table:rebuttal_linbp}
\vspace{-15pt}
\end{table}

==> table/eccv/rebuttal_multi_witness.tex <==
\begin{table}[h]
\captionsetup{font=scriptsize}
\begin{center}
\renewcommand{\arraystretch}{1}
\renewcommand{\tabcolsep}{1.1mm}
\scriptsize
\vspace{-10pt}
% \begin{tabular}{ ccccccccccc } 
% \Xhline{2\arrayrulewidth}
% \multirow{2}{*}{Witness}  & \multicolumn{10}{c}{Target} \\ \cline{2-11}
%                         & Res18	&Res50  &Res101 &VGG19	&DN121	&IncV3	&ViT-T	&ViT-S	&ViT-B	&SWIN \\\Xhline{2\arrayrulewidth}
% % Res18  	                & 79.82	&88.07	&78.20 &67.85	&78.45	&55.22	&31.07	&24.39	&20.48	&32.25     \\ 
% % Res18+IncV3+ViT-B	    & 58.67	&75.11	&61.50 &52.46	&66.95	&47.76	&28.76	&22.43	&\gc{20.53}	&29.51     \\ \hline
% Res50  	                & 54.13	&71.41	&61.13 &50.06	&59.56	&40.84	&26.25	&22.19	&19.28	&25.30     \\ 
% Res50+IncV3+ViT-S	    & 51.21	&66.25	&54.54 &48.65	&\gc{59.82}	&\gc{44.17}	&\gc{28.31}	&\gc{23.86}	&\gc{19.53}	&\gc{25.55}     \\
% \Xhline{2\arrayrulewidth}
% \end{tabular}
\begin{tabular}{ cccccccc } 
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Witness}  & \multicolumn{7}{c}{Target} \\ \cline{2-8}
                        & Res18	&Res50  &VGG19	&DN121	&IncV3	&ViT-S	&SWIN \\\Xhline{2\arrayrulewidth}
% Res18  	                & 79.82	&88.07	&78.20 &67.85	&78.45	&55.22	&31.07	&24.39	&20.48	&32.25     \\ 
% Res18+IncV3+ViT-B	    & 58.67	&75.11	&61.50 &52.46	&66.95	&47.76	&28.76	&22.43	&\gc{20.53}	&29.51     \\ \hline
Res50  	                & 54.13	&71.41	&50.06	&59.56	&40.84	&22.19	&25.30     \\ 
Res50+IncV3+ViT-S	    & 51.21	&66.25	&48.65	&\gc{59.82}	&\gc{44.17}	&\gc{23.86}	&\gc{25.55}     \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\vspace{-20pt}
\caption{\mbox{Aligning Res50 using witness models with different architectures.}}
\label{table:rebuttal_multi_witness}
\vspace{-13pt}
\end{table}
